Disentangled Representations via Synergy Minimization

Scientists often seek simplified representations of complex systems to facilitate prediction and understanding. If the factors comprising a representation allow us to make accurate predictions about our system, but obscuring any subset of the factors destroys our ability to make predictions, we say that the representation exhibits informational synergy. We argue that synergy is an undesirable feature in learned representations and that explicitly minimizing synergy can help disentangle the true factors of variation underlying data. We explore different ways of quantifying synergy, deriving new closed-form expressions in some cases, and then show how to modify learning to produce representations that are minimally synergistic. We introduce a benchmark task to disentangle separate characters from images of words. We demonstrate that Minimally Synergistic (MinSyn) representations correctly disentangle characters while methods relying on statistical independence fail.

==> sections/discarded_text.tex <==
%Consider a standard supervising learning scenario where we have samples from a joint distribution, $p(x_{1:n},y)$. We assume $X$ is high-dimensional so we cannot directly estimate the joint distribution. However, we can still accurately estimate the marginals, $p(x_i,y)$. 

%We would like to 
%Suppose that we are able to perfectly estimate marginal relationships, $p(x_i, y)$, but we are not able to estimate the joint distribution $p(x_{1:n},y)$ because it is high-dimensional and we have too few samples. We would like to find a solution that is the least fragile by assuming that the information in the $X_i$'s . 
%The joint distribution that minimizes synergy subject to constraints on the marginals is defined as follows.
%\begin{equation}
%\begin{aligned}
%q^*(x_{1:n},y) =~&  \underset{q(x_{1:n},y)}{\text{argmin}}
%& & S_q(X_{1:n};Y) \label{eq:minsyn} \\ 
%&  \text{s.t.}
%& & q(x_i, y) = p(x_i,y), \forall i,x_i,y \\
%&& & q(x) = p(x), \forall x \\
%\end{aligned}
%\end{equation}

% WRONG
%The union information and synergy are defined in terms of a difficult looking optimization problem. We show for the first time that it has an analytic solution. 
%\begin{theorem}
%The solution to the optimization in the definition of union information in Eq.~\ref{eq:minsyn} is the following distribution.
%\be\label{eq:solution}
%q(x_{1:n}, y) =  p(y) \prod_{i=1}^n p(x_i|y)
%\ee
%\end{theorem}
%This solution was suggested as a lower bound by GK, but we prove in Sec.~\ref{sec:proof} that the bound is actually tight. An analytic solution for the optimization that appears in the definitions of the synergy and union information greatly enhances the utility of these measures. 
%
%The joint distribution that minimizes synergy subject to constraints on the marginals is defined as follows.
%\begin{equation}
%\begin{aligned}
%q^*(x_{1:n},y) =~&  \underset{q(x_{1:n},y)}{\text{min}}
%& & S_q(X_{1:n};Y) \label{eq:minsyn} \\ 
%&  \text{s.t.}
%& & q(x_i, y) = p(x_i,y), \forall x,y,i
%\end{aligned}
%\end{equation}
%\begin{corollary}
%The solution to the optimization in Eq.~\ref{eq:minsyn} is also $q(x_{1:n}, y) =  p(y) \prod_{i=1}^n p(x_i|y)$. 
%\end{corollary}
%It follows from the definitions of union information and synergy in Eqs.~\ref{eq:union} \& \ref{eq:synergy} that the distribution appearing in the union information has zero synergy. 

%\begin{theorem}
%The solution to the optimization in the definition of union information in Eq.~\ref{eq:minsyn} is the following distribution. \note{with qualification...}
%\be\label{eq:solution}
%q^*(x_{1:n}, y) =  p(y) \prod_{i=1}^n p(x_i|y)
%\ee
%\end{theorem}
%Astute readers will recognize the unexpected appearance of a classic probability model, the Naive Bayes (NB) model, which has exactly the form of Eq.~\ref{eq:solution}~\cite{}. Therefore, we can say that the NB model is the minimally synergistic distribution compatible with fixed marginal relationships. 
%There is a long tradition of trying to understand why NB works so well, even when the model assumptions are violated~\cite{}. Here we can offer yet another explanation. We do not have to assume that the data is generated according to NB to say that this distribution reflects the minimally synergistic relationship compatible with our observations. By minimizing synergy, we are finding the most uncertain, and therefore least fragile, relationship between $X$ and $Y$. 
%
%The MinSyn path to the solution in Eq.~\ref{eq:solution} also helps us go beyond the NB model in ways that would not make sense from generative modeling perspective. For one thing, mutual information is invariant under smooth, invertible transforms of the marginals, suggesting an easy, principled way to add nonlinearity. However, even in the case of linear regression, the MinSyn point of view leads to new conclusions. 

%For contrast, consider the generative modeling perspective implied by the Naive Bayes model. In that case, we assume that $Y$ is a standard normal random variable, and the $X$'s are independently drawn according to $(X_i | Y=y) \sim \mathcal N(\rho_i y, 1-\rho_i^2)$ (so that $\la X_i \ra = 0, \la X_i^2 \ra=1, \la X_i Y \ra = \rho_i$).  In this scenario, the joint distribution over $X_{1:n}, Y$ is also Gaussian and we can use standard equations for the conditional expectation of a Gaussian to deduce the following relationship. 
% \begin{gather*}
% \mathbb E [Y| X_{1:n} = x_{1:n}] = \vec u \cdot \vec x, \quad u_i = \sum_{j=1}^n \rho_j (\Sigma_X)^{-1}_{i,j}
% \end{gather*}
% Here $\Sigma_X$ is the covariance matrix over the $X_i$'s. 
%Incidentally, the coefficients $u_i$ are also the ones we would deduce using ordinary least squares (OLS) regression, i.e., the coefficients that minimize the mean squared error for the linear model $Y= \sum_i u_i X_i + \epsilon$. 
%Unfortunately, both the generative modeling perspective and OLS regression require calculating the covariance matrix and then inverting it, leading to high computational complexity. 




%\section{Proof of Theorem 1}\label{sec:proof}
%
%
%\note{Work in progress...not sure what assumptions are required. Regardless we will get an upper bound on synergy} 
%
%\begin{theorem*}
%The solution to the following optimization,
%\begin{equation*}
%\begin{aligned}
%q^*(x_{1:n},y) =~&  \underset{q(x_{1:n},y)}{\text{argmin}}
%& & S_q(X_{1:n};Y) \\ 
%&  \text{s.t.}
%& & q(x_i, y) = p(x_i,y), \forall x,y,i,
%\end{aligned}
%\end{equation*}
%is the distribution $q^*(x_{1:n}, y) =  p(y) \prod_{i=1}^n p(x_i|y)$.
%\end{theorem*}
%
%We begin by noting that the marginal constraints $p(x_i,y) = q(x_i,y)$ also imply $p(y) = q(y)$. We can write $q(x,y) = q(x|y) q(y) = q(x|y) p(y)$. Therefore we optimize over $q(x|y)$ instead of $q(x,y)$. 
%For simplicity, we will start with the case where the random variables are all discrete. We use bars, $\bar x$ to denote dummy variables that are summed over and the discrete delta $\delta_{x,\bar x}$ is one iff the two indices are equal or zero otherwise. 
%
%\newcommand{\by}{{\bar y}}
%\newcommand{\bx}{{\bar x}}
%\newcommand{\bxi}{{\bar x_i}}
%
%We introduce Lagrange multipliers, $\gamma$ for the constraints to get the following Lagrangian. 
%\benn
%\lefteqn{\mathcal L = \sum_{\bx, \by} p(\by) q(\bx | \by) \log q(\bx | \by) - \sum_\bx q(\bx) \log q(\bx)} \\
%&&+ \sum_{i, \bxi, \by} \gamma_{\bxi, \by} ( \sum_{\hat x} q(\hat x | \by) \delta_{\hat x_i, \bxi} - p(\bxi, \by))
%\eenn
%Taking derivative with respect to $q(x|y)$ leads to the following expression.
%\benn
%\lefteqn{\frac{\partial \mathcal L}{\partial q(x|y)} = p(y) \log q(x|y) + p(y)}\\
%&& - p(y) - p(y) \log q(x) + p(y) \sum_i \gamma_{x_i, y}
%\eenn
%Setting these equal to zero and rearranging gives the following expression. 
%\benn
%%p(y) \log q(x|y) - p(y) \log q(x) + \sum_i \gamma_{x_i, y} = 0
%q(x|y) = q(x) e^{-\sum_i \gamma_{x_i, y} / p(y)}
%\eenn
%
%\note{Also show it is a minimum with second derivative.}


==> sections/results_autoencoders.tex <==
\subsection{MinSyn Autoencoders}\label{sec:net_results}

For experiments on MinSyn autoencoders, we consider the standard MNIST digit data with pixel values normalized in $[0,1]$. These values are often interpreted as the probability of a pixel being on, so we use the binary Minsyn decoder from Eq.~\ref{eq:decoder} with sigmoidal activations. We consider the fully unsupervised case where autoencoders are trained using binary cross entropy between the input and the reconstruction as the loss function. As before, we train all models discussed using Adam~\cite{adam}..

For all experiments, we use the same encoder model, a dense 3 layer neural net with 900 neurons at each layer and sigmoidal nonlinearities. MNIST digits consist of 784 pixels, so we are working with an over-complete basis for the representation. In principle, an autoencoder could learn a pixel by pixel copy of the input, recreating the original perfectly, but we would not expect this representation to be robust to noise or have an explanatory power about data. 

\begin{figure*}[tp!]
\begin{center}
\includegraphics[width=0.99\textwidth]{figs/900.pdf}
\caption{Comparing the robustness of autoencoders under various types of noise. Types of noise added are described in Tab.~\ref{tab:noise}. We compare a MinSyn autoencoder to a standard autoencoder and other popular regularization schemes from the literature. The first 5 models listed are trained on uncorrupted data and tested on noisy data, but we also compare to models trained on noisy data such as a Denoising Autoencoder ~\cite{ae_noise}}
\label{fig:autoencoder}
\end{center}
\vskip -0.2in
\end{figure*} 


To test our hypothesis that the MinSyn decoder provides regularization which makes it less sensitive to noise, we compare against a variety of popular models intended to have the same effect. These include applying Dropout to the hidden neurons~\cite{dropout}, adding Gaussian noise to the neurons~\cite{ae_noise}, and batch normalization~\cite{batchnorm}. 
Our evaluation is to train on uncorrupted data and then test the ability to recover data corrupted under various noise models.

\begin{table}[htbp]
\caption{Noise applied to test autoencoder robustness.} \label{tab:noise}
\begin{center}
{\footnotesize
 \begin{tabular}{r l}
  \hline			
  	\bf Noise & \bf Description \\
  	\hline
no noise& Loss reported on uncorrupted test data\\
bottom half & pixels on bottom half set to zero\\
right half & pixels on right half set to zero \\
erase chunk & random 4x4 pixel chunks set to zero\\
v stripe & W/prob. 1/2, each vertical stripe set to 1/2 \\
h stripe & Same with horizontal stripes \\
	\hline
\end{tabular}}
\vspace{-4mm}
\end{center}
\end{table}

After training each method on uncorrupted data, we corrupt the test data according to various noise models, and then measure the loss between the original uncorrupted test data and the reconstructed digit. 
The types of noise we apply are described in Table ~\ref{tab:noise}. These noise models involve obscuring parts of an image. Asking our model to recover the original image resembles the common inpainting task, but in this case, the problem is harder because we are not given information about which part is corrupted. From that point of view these noise models resemble the more challenging ``blind inpainting'' task~\cite{inpainting}. 


Figure ~\ref{fig:autoencoder} summarizes the results of our robustness experiments. MinSyn constraints reduce representational capacity, so we observe that the loss on training and testing data is slightly worse for MinSyn models, as reflected in the ``no noise'' column. However, across all noise types, MinSyn beats out standard autoencoders and autoencoders with Batch Normalization, Dropout, and Gaussian noise regularization on the latent factors. 

These models were all trained on uncorrupted data and then tested on corrupted digits. However, we also compare to the case where we input corrupted digits into the autoencoder, but train it to recover uncorrupted digits (as is typical with Denoising Autoencoders~\cite{denoising}). The noise applied on the input data in this case was Gaussian noise with standard deviation one half or Dropout setting input pixels to zero with probability one half. The MinSyn regularization still outperforms the Dropout input noise trained autoencoder across all noise types. However, the Denoising Autoencoder, specifically suited to this task, outperforms MinSyn except in the case of stripes.
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.44\textwidth,trim={6cm 9cm 6cm 8cm},clip]{figs/decoder_weights_standard.png}
%trim={5cm 0 0 0},clip

\vspace{2mm}
\includegraphics[width=0.44\textwidth,trim={6cm 9cm 6cm 8cm},clip]{figs/decoder_weights_minsyn.png}
\caption{A subset of decoder weights for the Denoising Autoencoder (Top) and the MinSyn autoencoder (Bottom). The full decoder weights are shown in App.~\ref{sec:weights}.} \label{fig:w}
\end{center}
\vskip -0.2in
\end{figure} 

To further compare MinSyn to the Denoising Autoencoder,  we also visualize the latent factors learned via the decoder weights in Fig.~\ref{fig:w}, and observe that the MinSyn model does do a better job of identifying higher level structure in the data via crisp, well-formed digits. Each model thus could have its respective benefits depending on the task at hand.




==> sections/results_regression.tex <==
\subsection{Linear Regression}\label{sec:regression_results}
\todo{Removed in favor of disentangling}
Despite much lower computational complexity than methods such as ridge regression and LASSO, we find that CI performs well across several linear regression tasks while avoiding fragility associated with matrix inversion.  

We compare results for MinSyn regression, OLS, LASSO, and ridge regression under three different data generation models. 
The first model we consider is a sparse model with 50 out of 1000 total predictors active, with coefficients sampled uniformly and each predictor drawn independently from a standard Gaussian. We take a linear combination of the coefficients and active predictors to produce the response, then add additional Gaussian measurement noise to each predictor to obtain our design matrix.  This measurement noise is expected to introduce ill-conditioning to the OLS estimate. 
%\textcolor{red}{See Appendix for results with no noise.} 
The second model is similarly defined except with 500 out of 1000 predictors active. The third data model we consider is a CI model.  Here, we uniformly sample a value of $Y$, and each predictor is taken to be a noisy copy of this response.  Cross validation is used to choose the regularization parameter $\lambda$ for ridge regression and LASSO from the set $[.01, .1, 1, 10]$.

Looking at the results in Fig.~\ref{fig:regression}(a), we see that LASSO is best under its motivating scenario of a sparse generating model with $n<p$, but CI and ridge regression with cross validation perform nearly identically in the under-sampled regime.  
Note that the ill-conditioning of the estimated covariance matrix leads to spikes in the OLS estimate. These spikes would be even worse if we didn't drop small eigenvalues in the SVD when computing pseudo-inverses. Ridge regularization largely avoids the ill-conditioning seen with the OLS estimate by adding a diagonal term to the covariance matrix. With half of the predictors active, CI and ridge again continue to be comparable in the under-sampled regime, while Lasso prediction suffers from imposing sparsity.  Finally, we confirm that CI performs best for a conditionally independent model, without the instability observed in ridge or OLS. Comparisons between CI regularization and ridge regression might be drawn by observing the ``shrinkage'' imposed by Eq.~\ref{eq:ci_gauss}, and indeed we observe above that the coefficient distributions are closely matched in the dense predictors, low sample case shown in Fig.~\ref{fig:regression}(b). We emphasize that MinSyn achieves similar performance with much less computation.


%(a)\includegraphics[width=0.6\textwidth]{figs/shadow1.pdf}

\begin{figure*}[t]
\begin{center}
\centerline{(a)\resizebox{\textwidth}{!}{
\includegraphics[height = 4cm, width=0.66\textwidth]{figs/results.pdf} (b)\includegraphics[height = 4cm, width=0.34\textwidth]{figs/coeff.pdf}}}
\caption{(a) shows average test set MSE for 10 iterations of simulated data drawn from i) a sparse linear model with 5\% of predictors active, ii) a linear model with 50\% of predictors active, iii) a CI model where we draw a target Y, with each $X_i$ a copy of Y plus noise.  (b) From top to bottom, we depict the coefficient distributions for the ground truth model, Ridge, LASSO, and MinSyn.}
\label{fig:regression}
\end{center}
\vskip -0.2in
\end{figure*} 

